Convolutional restricted Boltzmann machine aided Monte Carlo: An application to Ising and Kitaev models

Machine learning is becoming widely used in analyzing the thermodynamics of many-body condensed matter systems. Restricted Boltzmann Machine (RBM) aided Monte Carlo simulations have sparked interest recently, as they manage to speed up classical Monte Carlo simulations. Here we employ the Convolutional Restricted Boltzmann Machine (CRBM) method and show that its use helps to reduce the number of parameters to be learned drastically by taking advantage of translation invariance. Furthermore, we show that it is possible to train the CRBM at smaller lattice sizes, and apply it to larger lattice sizes. To demonstrate the efficiency of CRBM we apply it to the paradigmatic Ising and Kitaev models in two-dimensions.

==> FRBM_vs_CRBM.tex <==
In Sec.~\ref{sec:kitav_periodic} it was established that the FRBM had a worse performance for the Kitaev model than the CRBM. It was noted that the learned weights of the FRBM showed hardly any interaction in the z-direction. To further understand this effect the CRBM was trained again with a smaller kernel with size $1\times5\times5$. This kernel is compared in Fig.~\ref{fig:kitaev_CRBMvsFRBM} to one of the interaction terms of an FRBM trained with $8^2$ hidden units. When restricting the CRBM to just one kernel it learns the same pattern as the FRBM and accordingly performs similarly. Since the reduced CRBM no longer can capture the full interaction, it focuses on the stronger interaction in the z-direction and neglects the interaction in the x-y-direction. This explains why the FRBM with $8^2$ hidden units performs badly. The FRBM with $2\times8^2$ hidden units should be able to learn the interaction to the same degree as the the CRBM since a CRBM with kernel size $2\times5\times5$ can be mapped to a FRBM with $2\times8^2$ hidden units. The question that remains is why in this case the FRBM can not learn the interaction in the x-y-direction. To find an answer the learned $1\times5\times5$ CRBM kernel is duplicated to yield a kernel of size $2\times5\times5$. When this kernel is trained it does not learn the interaction in the z-direction as it gets trapped in the local minima where only the interaction in the x-y-direction are learned. We conclude that it is much easier for the FRBM to get stuck in local minima since it not only needs to learn the interaction but also needs to learn to be translationally invariant.
\begin{figure}
	\centering
	\subfloat{\includegraphics[width=0.5\textwidth]{images/kitaev_CRBMvsFRBM_kernel_L=8.png}}
	\caption{RBM weights trained at $T=0.18$ for both CRBM and FRBM. (left) Kernel of a CRBM trained with size $1\times5\times5$. (right) The 59 component in Fig.~\ref{fig:kitaev_FRBM_kernel}, which depicts one of the weights of the FRBM with a total of $8^2$ hidden units.}
	\label{fig:kitaev_CRBMvsFRBM}
\end{figure}


